RIS-Assisted Coverage Enhancement in Millimeter-Wave Cellular Networks

The use of millimeter-wave (mmWave) bandwidth is one key enabler to achieve the high data rates in the fifth-generation (5G) cellular systems. However, mmWave signals suffer from significant path loss due to high directivity and sensitivity to blockages, limiting its adoption within small-scale deployments. To enhance the coverage of mmWave communication in 5G and beyond, it is promising to deploy a large number of reconfigurable intelligent surfaces (RISs) that passively reflect mmWave signals towards desired directions. With this motivation, in this work we study the coverage of an RIS-assisted large-scale mmWave cellular network using stochastic geometry, and derive the peak reflection power expression of an RIS and the downlink signal-to-interference ratio (SIR) coverage expression in closed forms. These analytic results clarify the effectiveness of deploying RISs in the mmWave SIR coverage enhancement, while unveiling the major role of the density ratio between active base stations (BSs) and passive RISs. Furthermore, the results show that deploying passive reflectors is as effective as equipping BSs with more active antennas in the mmWave coverage enhancement. Simulation results confirm the tightness of the closed form expressions, corroborating our major findings based on the derived expressions.

==> Sections/2_2ref.tex <==
%In the conventional cellular networks, there are active BSs communicating with the UEs.
As shown in Fig. \ref{fig:Conven-1}, the UE communicates with the nearest BS. The PDF of the distance of the UE from the nearest BS, denoted by $r_0$, is obtained from the void probability in Poisson process of $\mathbb{R}^2$ like in \cite{PPP} as follows
\begin{equation}
    f_{r_0}(r_0)=2\pi \lambda_{BS} r_0 e^{-\lambda_{BS}\pi r_{0}^2}.
    \label{pdfR0}
\end{equation}

 The existing coverage analysis in \cite{REF} evaluated the conventional cellular networks for sub-6 GHz frequency bands. We exploit their analysis and modify it to introduce our baseline mm-Wave cellular networks. In general, as shown in Fig. \ref{fig:Conven-1}, there are two types of signal power sources. One which is the desired signal power received by the UE from the associated BS as the desired source, and another which is the interference signal power received by the UE from the interferer BSs. ne main difference in the mm-Wave cellular networks compared to the sub-6 GHz cellular networks, is that due to the mm-Wave propagation characteristics \cite{parkBW}, beamforming is used to converge the signal power in a specific direction towards a desired UE.
 Based on the \textit{Assumption 3} and the uniform planar square array (UPA) in 2-D world \cite{parkBW}, the active BSs which are equipped with $N$ isotropic elements are able to create single beam with beamwidth of 
 \begin{equation}
     \psi_\textbf{o}=\frac{2\pi}{\sqrt{N}}.
     \label{BW1}
 \end{equation}
 In addition, we assume that each interferer BS transmits with its main-lobe pointed at a random direction. Intuitively, it affects the density of interferer BSs as a modified homogeneous PPP, denoted by $\Phi_I$, with intensity of $\lambda_I$ given as
  \begin{equation}
      \lambda_I=\frac{\lambda_{BS}}{\sqrt{N}}.
      \label{lam_I}
  \end{equation}
 In other words, only a subset of interferer BSs in which their beamforming direction covers the desired UE are considered as the effective interferer BSs for the UE. \\
 
%
Let $\Gamma_\textbf{o}$ denote the SIR at an independent UE in the baseline mm-Wave cellular network. Consequently, the SIR can be obtained as
%\begin{equation}
    %\textbf{SINR}_\textbf{A}=\frac{P_s g_0 r_0^{-\alpha}}{\sigma_n^2+\sum\limits_{\substack{BS_i %\in \Phi_{I},\\ i\neq 0}} P_s g_i r_i^{-\alpha}},
 %   \label{S-A}
%\end{equation}
\begin{equation}
    {\Gamma}_\textbf{o}=\frac{P_s g_0 r_0^{-\alpha}}{\sum\limits_{\substack{BS_i \in \Phi_{I},\\ i\neq 0}} P_s g_i r_i^{-\alpha}},
    \label{S-A}
\end{equation}
where $g_i$ and $r_i$ are small-scale channel gain and the distance of the $i$th BS, denoted by $BS_i$, from the UE, respectively. $i=0$ indicates the nearest BS which is the associated BS. $\alpha$ is also the path-loss exponent of large-scale fading. \\

 The SIR coverage probability is the probability that the received SIR is larger than a threshold. Let $T$ denote the threshold and from \eqref{S-A}, the SIR coverage probability is given by 
     \begin{align}
    \Pr\left[\Gamma_\textbf{o}>T\right]=\mathbb{E}\left\{\Pr\left(\frac{P_s g_0 r_0^{-\alpha} }{\sum\limits_{BS_i \in \Phi_{I}} P_s g_i r_i^{-\alpha}}>T\right)\right\}.
    \label{eq213}
\end{align}
 \iffalse
    \begin{align}
    \Pr\left[\textbf{SINR}_\textbf{A}>T\right]=\mathbb{E}\left\{\Pr\left(\frac{P_s g_0 r_0^{-\alpha} }{\sigma_n^2+\sum\limits_{b_i \in \Phi_{I}} P_s g_i r_i^{-\alpha}}>T\right)\right\}.
    \label{eq213}
\end{align}
\fi
In other words, it is equivalent with the complementary cumulative distribution function (CCDF) of SIR. In order to simplify the analysis to find the closed-form expression of \eqref{eq213}, we utilize the following lemma.
\begin{lemma}
{\it (Power-Density Conversion:)} At one specific point, the received power of a homogeneous PPP $(\Phi)$ set of transmitters with transmit power of $P$ and intensity of $\lambda$ is equivalent with the received power of homogeneous PPP $(\tilde{\Phi})$ set of virtual transmitters with unit transmit power of 1 and intensity of $\tilde{\lambda}$ which is given as
\begin{equation}
    \tilde{\lambda}=P^{\frac{2}{\alpha}}\lambda.
\end{equation}
\label{lem1}
\end{lemma}
\begin{proof}
 The proof is given in Appendix \ref{AP1}.
\end{proof}

From \textit{Assumption 4}, we have $\forall i\rightarrow g_i\sim \exp (\mu)$. Therefore, utilizing Lemma 1, we have $\Phi_{BS}\rightarrow \tilde{\Phi}_{BS}$ and $\Phi_{I}\rightarrow \tilde{\Phi}_{I}$; and \eqref{eq213} can be re-written as
\begin{align}
    \Pr\left[\Gamma_\textbf{o}>T\right]=\mathop{\mathbb{E}}\left\{\Pr\left(\frac{\tilde{g}_0 r_0^{-\alpha} }{\sum\limits_{\substack{BS_i \in \tilde{\Phi}_{I}\\i\neq 0}} \tilde{g}_i r_i^{-\alpha}}>T\right)\right\},
    \label{eq41}
\end{align}
where
\begin{equation}
   \left\{\begin{array}{l}
        \tilde{\lambda}_{BS}=\left(\frac{P_s}{\mu}\right)^{-\frac{2}{\alpha}} \lambda_{BS} \\
        \tilde{\lambda}_I=\left(\frac{P_s}{\mu}\right)^{-\frac{2}{\alpha}} \frac{\lambda_{BS}}{\sqrt{N}}\\
                \tilde{g}_i\sim \exp (1) 
   \end{array} \right. . 
  \label{rt32}
\end{equation}

After analysis given in Appendix \ref{AP0}, we have the following proposition.
\begin{proposition}
The coverage probability of a typical randomly located UE in the baseline
mm-Wave cellular network model is given by
\begin{align}
    \Pr\left[\Gamma_\textbf{o}>T\right]&=
    \frac{\tilde{\lambda}_{BS}}{\left(\tilde{\lambda}_{BS}+\tilde{\lambda}_{I}T^{\frac{2}{\alpha}}
         \int_{T^{-\frac{2}{\alpha}}}^\infty \frac{1}{1+u^{\frac{\alpha}{2}}}du\right)}
         \label{q4}
\end{align}
\end{proposition}

\begin{proof}
 The proof is given in Appendix \ref{AP0}.
\end{proof}

By substituting \eqref{rt32} in \eqref{q4}, we have

\begin{align}
    \Pr\left[\Gamma_\textbf{o}>T\right]&=
         \frac{1}{\left(1+\frac{1}{\sqrt{N}}T^{\frac{2}{\alpha}}
         \int_{T^{-\frac{2}{\alpha}}}^\infty \frac{1}{1+u^{\frac{\alpha}{2}}}du\right)}
         \label{q2}
\end{align}





==> Subs/AP2.tex <==
 The SINR coverage probability is the probability that the received SINR is larger than a threshold. Let $T$ denote the threshold and from \eqref{S-A}, the SINR coverage probability is given by 
    \begin{align}
    \Pr\left[\textbf{SINR}_\textbf{A}>T\right]=\mathbb{E}\left\{\Pr\left(\frac{P_s g_0 r_0^{-\alpha} }{\sigma_n^2+\sum\limits_{b_i \in \Phi_{I}} P_s g_i r_i^{-\alpha}}>T\right)\right\}.
    \label{eq213}
\end{align}
In other words, it is equivalent with the complementary cumulative distribution function (CCDF) of SINR. In order to simplify the analysis to find the closed-form expression of \eqref{eq213}, we utilize the following lemma.
\begin{lemma}
{\it Power-density conversion:} At one specific point, the received power of a homogeneous PPP $\Phi$ set of transmitters with transmit power of $P$ and intensity of $\lambda$ is equivalent with the received power of homogeneous PPP $\tilde{\Phi}$ set of virtual transmitters with unit transmit power and intensity of $\tilde{\lambda}$ given as follows 
\begin{equation}
    \tilde{\lambda}=P^{\frac{2}{\alpha}}\lambda.
\end{equation}
\end{lemma}
\begin{proof}
 The proof is given in Appendix \ref{AP1}.
\end{proof}
Consequently, we can assume $\Phi_{BS}\rightarrow \tilde{\Phi}_{BS}$ and $\Phi_{I}\rightarrow \tilde{\Phi}_{I}$ where 
\begin{equation}
   \left\{\begin{array}{l}
        \tilde{\lambda}_{BS}=\left(\frac{P_s}{\mu}\right)^{-\frac{2}{\alpha}} \lambda_{BS} \\
        \tilde{g}_i\sim \exp (1) \\
   \end{array} \right. . 
  \label{rt32}
\end{equation}
For notational simplicity, we omit the tilde symbol from $\tilde{g}_i$ and consider it as $g_i$ in the rest of analysis while keeping its characteristic changes in \eqref{rt32}. Thus, \eqref{eq213} becomes
\begin{align}
    \Pr&\left[\textbf{SINR}_\textbf{A}>T\right]=\mathop{\mathbb{E}}\left\{\Pr\left(\frac{g_0 r_0^{-\alpha} }{\sigma_n^2+\sum\limits_{\substack{b_i \in \tilde{\Phi}_{I}\\i\neq 0}} g_i r_i^{-\alpha}}>T\right)\right\}\nonumber\\
    &\hspace{5mm}
    =\mathop{\mathbb{E}}\limits_{\substack{g_0\\g_i\\r_i\\r_0}}\left\{\Pr\left(g_0> Tr_0^{\alpha}\left[ \sigma_n^2+\sum\limits_{\substack{b_i \in \tilde{\Phi}_{I}\\i\neq 0}} g_i r_i^{-\alpha}\right]\right)\right\}.
    \label{eq214}
\end{align}
Since $g_0\sim \exp (1)$, we have $\Pr (g_0>x)=1-F_{g_0}(x)=e^{-x}$, \eqref{eq214} becomes

\begin{align}
    \Pr&\left[\textbf{SINR}_\textbf{A}>T\right]=\nonumber\\
    &\hspace{5mm}
    \mathop{\mathbb{E}}\limits_{\substack{g_i\\r_i\\r_0}}\left\{\exp\left(- Tr_0^{\alpha}\left[ \sigma_n^2+\sum\limits_{\substack{b_i \in \tilde{\Phi}_{I}\\i\neq 0}} g_i r_i^{-\alpha}\right]\right)\right\}\nonumber\\
    &\hspace{5mm}
    \mathop{\mathbb{E}}\limits_{\substack{r_i\\r_0}}\left\{ e^{- Tr_0^{\alpha}} \times \prod\limits_{\substack{b_i \in \tilde{\Phi}_{I}\\i\neq 0}} \mathop{\mathbb{E}}\limits_{\substack{g_i}}\left\{\exp \left( -g_iT\left[\frac{r_0}{r_i}\right]^\alpha\right)\right\}\right\}.
    \label{eq216}
\end{align}
Since, $g_i \sim \exp (1)$, we have $\mathbb{E}\left\{e^{-g_ix}\right\}=\left[1+x\right]$. Therefore, \eqref{eq216} becomes
\begin{align}
    \Pr&\left[\textbf{SINR}_\textbf{A}>T\right]=\nonumber\\
    &\hspace{5mm}
    \mathop{\mathbb{E}}\limits_{\substack{r_0}}\left\{ e^{- Tr_0^{\alpha}} \times \mathop{\mathbb{E}}\limits_{\substack{r_i}}\left\{\prod\limits_{\substack{b_i \in \tilde{\Phi}_{I}\\i\neq 0}} \left(1+T\left[\frac{r_0}{r_i}\right]^\alpha\right)^{-1}\right\}\right\}.
    \label{eq217}
\end{align}
